Stochastic Bandits with Vector Losses: Minimizing $\ell^\infty$-Norm of Relative Losses

Multi-armed bandits are widely applied in scenarios like recommender systems, for which the goal is to maximize the click rate. However, more factors should be considered, e.g., user stickiness, user growth rate, user experience assessment, etc. In this paper, we model this situation as a problem of $K$-armed bandit with multiple losses. We define relative loss vector of an arm where the $i$-th entry compares the arm and the optimal arm with respect to the $i$-th loss. We study two goals: (a) finding the arm with the minimum $\ell^\infty$-norm of relative losses with a given confidence level (which refers to fixed-confidence best-arm identification); (b) minimizing the $\ell^\infty$-norm of cumulative relative losses (which refers to regret minimization). For goal (a), we derive a problem-dependent sample complexity lower bound and discuss how to achieve matching algorithms. For goal (b), we provide a regret lower bound of $\Omega(T^{2/3})$ and provide a matching algorithm.

==> appendices/app_cg.tex <==
\section{Proof of Theorem~\ref{thm:cg}}\label{app:cg}



% To begin with, we first prove the following lemma.
% \begin{lemma}\label{lemma:concentration}
% For any given $k,l\in[K]$ with $k\neq l$, if for all $i\in \left\{1,2\right\}$, we have $\abs{\hloss{i}{j}- \loss{i}{j}}\leq \epsilon$ for $j\in\{k,l,\star_1,\star_2\}$, then we have
% \begin{align*}
% \abs{\hclstar{k}{l}-\clstar{k}{l}} \leq 2\epsilon,
% \end{align*}
% and therefore, $\forall i\in \{1,2\}$,
% \begin{align*}
% \abs{\hcloss{i}{k}{l}-\closs{i}{k}{l}} \leq 3\epsilon.
% \end{align*}
% \end{lemma}

% \begin{proof}
% We have
% \begin{align*}
% \hclstar{k}{l} &= \max_{i\in\{1,2\}}\min_{\alpha\in[0,1]} (\alpha \hlstar{i}{k}+(1-\alpha)\hlstar{i}{l})\leq \max_{i\in\{1,2\}}\min_{\alpha\in[0,1]} \left(\alpha (\lstar{i}{k}+2\epsilon) +(1-\alpha)(\lstar{i}{l}+2\epsilon)\right)\\
% &= \max_{i\in\{1,2\}}\min_{\alpha\in[0,1]} (\alpha \lstar{i}{k}+(1-\alpha)\lstar{i}{l})+2\epsilon = \clstar{k}{l}+2\epsilon.
% \end{align*}
% Similarly we have $\hclstar{k}{l}\geq \clstar{k}{l}-2\epsilon$. The second inequality is trivial by definition.
% \end{proof}

We first show that the empirical estimation is valid with high probability at each round. Specifically, we have the following lemma.

\begin{lemma}\label{lemma:conc}
Define the following event:
\begin{align*}
    E_{1,t}\triangleq \left\{\forall k\in[K],i\in [d]: \abs{\hloss{i}{k}- \loss{i}{k}}\leq \sqrt{\dfrac{2\log(t)}{N_{k}}} \right\},
\end{align*}
where $N_{k}$ denotes the number of pulls of arm $k$. This event will happen with probability at least $1- dK/t^2$, that is:
\begin{align*}
    \PP {E_{1,t}} \geq 1- \frac{dK}{t^2}
\end{align*}
\end{lemma}

\begin{proof}
This is the a direct application of the Hoeffding's Inequality with the union bound.
\end{proof}




With the Lemma above, we proceed to show that $\LCB(\blstar{}{})$ is a valid approximation for $\blstar{}{}$. Concretely, we have the following lemma.

\begin{lemma}
Assume $E_{1,t}$ holds, we have,
\begin{align*}
    \LCB_t(\blstar{}{})_{i,k} \le \lstar{i}{k} \le \LCB_t(\blstar{}{})_{i,k} + 2\sqrt{\frac{2\log(t)}{N_{t,k}}} +2 \sqrt{\frac{2\log(t)}{N}}.
\end{align*}
\end{lemma}
\begin{proof}
This is a easy deduction of Lemma~\ref{lemma:conc}.
\end{proof}


% We recall the theorem below.
% \restatecg*


% \begin{proof}
% Recall the event $E_{1,t}$ defined in Lemma~\ref{lemma:conc}, we can decompose the regret as follows.
% \begin{align}
%   &\EE{R_{\CG}(T)} = \EE{\max_{i\in[d]}\sum_{t=1}^T\lstar{i}{\cA_t}} - \wlstar{\bomega^\star}T \nonumber\\
%     \leq& KN+ \EE{\max_{i\in[d]}\sum_{t\geq KN}\lstar{i}{\cA_t}\II{\neg E_{1,t}}} + \EE{\max_{i\in[d]}\sum_{t\geq KN}\lstar{i}{\cA_t}\II{E_{1,t}}} - \wlstar{\bomega^\star}T\:.
% \end{align}

% For the second term, due to Lemma~\ref{lemma:conc}, we have
% \begin{align*}
%     \EE{\max_{i\in[d]}\sum_{t\geq KN}\lstar{i}{\cA_t}\II{\neg E_{1,t}}}\leq \EE{\sum_{t\geq KN}\II{\neg E_{1,t}}}\leq \sum_{t\geq KN}\frac{dK}{t^2} \leq \frac{\pi^2dK}{6}\,.
% \end{align*}

% For the third term, we first decompose the regret into a term related to strategies of both players and the tracking error. 
% \begingroup
% \allowdisplaybreaks
% \begin{align}
%     &\EE{\max_{i\in[d]}\sum_{t\geq KN}\lstar{i}{\cA_t}\II{E_{1,t}}}  \leq \EE{\max_{i\in[d]} \sum_{k=1}^K \sum_{t= KN+1}^T \lstar{i}{k}\II{E_{1,t},\cA_t = k}}\nonumber\\
%     \leq& \EE{\max_{i\in[d]} \sum_{k=1}^K\sum_{t=KN+1}^{T} \omega_{t,k}\lstar{i}{k}\II{E_{1,t}}} + \EE{\max_{i\in[d]}\sum_{k=1}^K \sum_{t=1+KN}^{T}\left(\II{\cA_t = k}- \omega_{t,k}\right)\II{E_{1,t}}\lstar{i}{k}}\nonumber\\
%      \leq& \EE{\max_{i\in[d]} \sum_{k=1}^K\sum_{t=KN+1}^{T} \omega_{t,k}\lstar{i}{k}\II{E_{1,t}}}+\EE{\max_{i\in[d]}\sum_{k=1}^K \sum_{t=1+KN}^{T}\left(\II{\cA_t = k}- \omega_{t,k}\right)\lstar{i}{k}} \nonumber\\ 
%      &+ \EE{\max_{i\in[d]}\sum_{k=1}^K \sum_{t=1+KN}^{T}\left( \omega_{t,k}-\II{\cA_t = k}\right)\lstar{i}{k}\II{\neg E_{1,t}}}\nonumber\\
%     \leq &\EE{\sum_{t=KN+1}^{T} \max_{\bx\in \Sigma^d} \bx^\top \blstar{}{} \bomega_t\II{E_{1,t}}} + K + \frac{\pi^2K}{6}\label{eq:tracking}\:,
% \end{align}
% where~\eqref{eq:tracking} adopts Lemma~15 by~\cite{garivier2016tracknstop}. Thus the first term in~\eqref{eq:tracking} can be further estimated. 
% \begin{align}
%     &\EE{\sum_{t=KN+1}^{T} \max_{\bx\in \Sigma^d} \bx^\top \blstar{}{} \bomega_t\II{E_{1,t}}}\nonumber\\
%     \leq& \EE{\sum_{t=KN+1}^{T}  \max_{\bx\in \Sigma^d} \bx^\top \LCB(\blstar{}{}) \bomega_t\II{E_{1,t}}} + \EE{2\sum_{t=KN+1}^{T}\sum_{k=1}^K \left(\sqrt{\frac{2\log(T)}{N_{t,k}}} \right)\omega_{t,k}}\nonumber\\ 
%     &+ 2T\sqrt{\frac{2\log(T)}{N}} \nonumber\\
%     \leq& \EE{\sum_{t=KN+1}^{T}  \max_{\bx\in \Sigma^d} \bx^\top \LCB(\blstar{}{}) \bomega_t\II{E_{1,t}}} + 2(K^2+\sqrt{2KT})\sqrt{2\log(T)}\nonumber\\ 
%     &+ 2T\sqrt{\frac{2\log(T)}{N}} \label{eq:track2}\\
%     \leq& \EE{\sum_{t=KN+1}^{T}  \max_{\bx\in \Sigma^d} \bx^\top \LCB(\blstar{}{}) \bomega_t} + 2(K^2+\sqrt{2KT})\sqrt{2\log(T)}\nonumber\\ 
%     &+ 2T\sqrt{\frac{2\log(T)}{N}} + \frac{\pi^2}{6}K\nonumber\\
%     \leq& \EE{\sum_{t=KN+1}^{T}  \bx_t^\top \LCB(\blstar{}{}) \bomega^\star} + \sqrt{T} + 2(K^2+\sqrt{2KT})\sqrt{2\log(T)}\nonumber\\
%     &+ 2T\sqrt{\frac{2\log(T)}{N}} + \frac{\pi^2}{6}K\label{eq:orcreg}\:,
% \end{align}  
% where~\eqref{eq:track2} adopts Lemma~9 by \cite{degenne2019game} and~\eqref{eq:orcreg} uses the fact that $\cL$ has regret $\sqrt{T}$. Now we are only left to bound the first term in~\eqref{eq:orcreg}.
% \begin{align}
%     &\EE{\sum_{t=KN+1}^{T}  \bx_t^\top \LCB(\blstar{}{}) \bomega^\star}\nonumber\\
%     \leq & \EE{\sum_{t=KN+1}^{T}  \bx_t^\top \blstar{}{} \bomega^\star} + \frac{\pi^2}{6}K\nonumber\\
%     \leq & (T-KN)  \max_{\bx\in \Sigma^d} \bx^\top \blstar{}{} \bomega^\star +  \frac{\pi^2}{6}K\nonumber\\
%     = & (T-KN)\wlstar{\bomega^\star} + \frac{\pi^2}{6}K\nonumber\:,
% \end{align}
% \endgroup
% Therefore, aggregating all the terms above we have the regret is upper bounded by $\cO(KN+T\sqrt{\log(T)/N})=\tcO(T^{2/3})$ by setting $N=(K^2T^2\log(T))^{1/3}$.
% \end{proof}

==> appendices/app_lb.tex <==
\section{Proof of Theorem~\ref{thm:lb}}\label{app:lb}

We prove the lower bound in this section, namely Theorem~\ref{thm:lb} as recalled as follow.

\restatelb*


\begin{proof}
    Let $\epsilon > 0$ be a constant, we consider a bandit model $\bnu$ with the following 2-dimensional loss vectors:
    \begin{gather*}
    \bell_1 = \left(\frac{1}{4},\frac{3}{4}\right), \bell_2 = \left(\frac{3}{4},\frac{1}{4}\right), \bell_3 = \left( \frac{3-\epsilon}{8}, \frac{3+\epsilon}{8}\right), \bell_4 = \left(  \frac{3+\epsilon}{8},  \frac{3-\epsilon}{8}\right)\,,
    \end{gather*}
    where the losses are Gaussian distributions with variance 1 and expectation of the indicated value. 

    Since there is a symmetry between arm 3 and arm 4. Without loss of generality, we assume for the given algorithm $\cA$ under consideration, that $\mathbb{E}_{\cA,\bnu}\left[N_3\right]\leq \mathbb{E}_{\cA,\bnu}\left[N_4\right]$.
    Then according to the assumption between $N_3$ and $N_4$, we consider an alternative bandit model $\bnu'$ with the following loss vectors,
    \begin{gather*}
        \bell'_1 = \left(\frac{1-\epsilon}{4},\frac{3}{4}\right), \bell'_2 = \left(\frac{3}{4},\frac{1}{4}\right), \bell'_3 = \left( \frac{3-\epsilon}{8}, \frac{3+\epsilon}{8}\right), \bell'_4 = \left(  \frac{3+\epsilon}{8},  \frac{3-\epsilon}{8}\right)\,.
    \end{gather*}
    ~\\
    % \textbf{Claim 1 for bandit model $\bnu'$:} 
    % \[
    %     \text{The optimal combination } \omega^\star_{\bnu'} = (0,0,1,0)\,.
    % \]

    The optimal arms for each loss are $\star_1 = 1$, $\star_2 = 2$.
    \begin{align*}
        \omega^\star_\bnu 
        &\eqdef \argmin_{\bomega\in\Sigma_K} \max_{i\in[d]} \left\{\bomega^\top \bloss{i}_{\bnu}-\loss{i}{\star_i,\bnu}\right\} \\
        &= \argmin_{\bomega\in\Sigma_K} \max \biggl\{ \frac{(2+\epsilon)\omega_2}{4} + \frac{(1+\epsilon)\omega_3}{8} + \frac{(1+3\epsilon)\omega_4}{8},\\
        &\qquad\qquad \frac{\omega_1}{2} + \frac{(1+\epsilon)\omega_3}{8} + \frac{(1-\epsilon)\omega_4}{8} \biggr\}\\
        &=\argmin_{\bomega\in\Sigma_K} \max \left\{ \frac{(2+\epsilon)\omega_2 }{4} + \frac{\epsilon \omega_4}{2}, \frac{\omega_1}{2} \right\}\\
        &=(0,0,1,0).
    \end{align*}
    ~\\
    % \textbf{Claim 2 for bandit model $\bnu'$:}
    %     \[
    %         \text{If } \epsilon < \frac{1}{6}: R_{\bnu'}(T)\geq \frac{1}{144}N_1 + \frac{1}{6}N_2 +   \frac{\epsilon}{12}(T - N_3)\,.
    %     \]
    $\text{For } \epsilon < \frac{1}{6}:$
    \begingroup
    \allowdisplaybreaks
    \begin{align*}
        R_{\bnu'}(T) 
        &\triangleq \max_{i\in [d]}\left(\Loss{i}{}- \loss{i}{\bomega^\star}T\right) \\
        &= \max \biggl\{  \frac{(1-\epsilon)N_1}{4} + \frac{3N_2}{4} + \frac{(3-\epsilon)N_3}{8} + \frac{(3+\epsilon)N_4}{8} - \frac{3-\epsilon}{8}T,\\
        &\qquad\qquad \frac{3N_1}{4} + \frac{N_2}{4} + \frac{(3+\epsilon)N_3}{8} + \frac{(3-\epsilon)N_4}{8} - \frac{3+\epsilon}{8}T \biggr\}\\
        &= \max  \biggl\{  -\frac{(1+\epsilon)N_1}{8} + \frac{(3+\epsilon)N_2}{8}  + \frac{\epsilon N_4}{4},\\
        &\qquad\qquad \frac{(3-\epsilon)N_1}{8} - \frac{(1+\epsilon)N_2}{8}  - \frac{\epsilon N_4}{4} \biggr\}\\
        &\geq \frac{2}{3} \left(   -\frac{(1+\epsilon)N_1}{8} + \frac{(3+\epsilon)N_2}{8}  + \frac{\epsilon N_4}{4} \right) \\
        &+ \frac{1}{3} \left(  \frac{(3-\epsilon)N_1}{8} - \frac{(1+\epsilon)N_2}{8}  - \frac{\epsilon N_4}{4}  \right)\\
        &\geq \frac{1}{48}N_1 + \frac{5}{24}N_2 + \frac{\epsilon}{12} N_4 \\
        &= (\frac{1}{48} - \frac{\epsilon}{12}  )N_1 + (\frac{5}{24} - \frac{\epsilon}{12} )N_2 +  \frac{\epsilon}{12}(T - N_3) \\
        &\geq \frac{1}{144}N_1 + \frac{1}{6}N_2 +   \frac{\epsilon}{12}(T - N_3)\,.
    \end{align*}
    \endgroup
    ~\\
    So we have the following regret for the bandit model $\bnu'$,
    \begin{align}
        \mathbb{E}\left[R_{\cA,\bnu'}(T)\right] 
        &\geq  \frac{1}{144}\mathbb{E}_{\cA,\bnu'}\left[N_1\right] + \frac{\epsilon}{12} \left(T - \mathbb{E}_{\cA,\bnu'}\left[N_3\right]\right)\,.\label{eq:lbalter}
    \end{align}
    According to the inequality (6) by~\cite{garivier2018explore}, we have,
    \begin{align*}
    \frac{\epsilon^2}{2} \mathbb{E}_{\cA,\bnu'}\left[N_1\right]\geq \text{kl} \left(\frac{ \mathbb{E}_{\cA,\bnu'}\left[N_3\right]}{T},\frac{ \mathbb{E}_{\cA,\bnu}\left[N_3\right]}{T}  \right) \geq 2 \left( \frac{ \mathbb{E}_{\cA,\bnu}\left[N_3\right]}{T} - \frac{ \mathbb{E}_{\cA,\bnu'}\left[N_3\right]}{T} \right)^2\,.
    \end{align*}
    Therefore,
    \begin{align*}
        \mathbb{E}_{\cA,\bnu'}\left[N_3\right] \leq \frac{\epsilon}{2} T \s{\mathbb{E}_{\cA,\bnu'}\left[N_1\right]} + \mathbb{E}_{\cA,\bnu}\left[N_3\right]
    \end{align*}
    Furthermore with $\mathbb{E}_{\cA,\bnu}\left[N_3\right] \leq T/2$, and according to our assumption,
    \begin{align*}
    \mathbb{E}\left[R_{\cA,\bnu'}(T)\right]
    &\geq\frac{1}{144}\mathbb{E}_{\cA,\bnu'}\left[N_1\right] + \frac{\epsilon}{12} \left(T - \mathbb{E}_{\cA,\bnu'}\left[N_3\right]\right)\\
    &\geq \frac{1}{144}\mathbb{E}_{\cA,\bnu'}\left[N_1\right]  + \frac{\epsilon}{12} T - \frac{\epsilon^2}{24}T\s{\mathbb{E}_{\cA,\bnu'}\left[N_1\right]} - \frac{\epsilon}{12} \mathbb{E}_{\cA,\bnu}\left[N_3\right] \\
    &\geq \frac{1}{144}\mathbb{E}_{\cA,\bnu'}\left[N_1\right]  + \frac{\epsilon}{24} T - \frac{\epsilon^2}{24}T\s{\mathbb{E}_{\cA,\bnu'}\left[N_1\right]} 
    \end{align*}
    Take $\epsilon = T^{-1/3}/2 < 1/6$, we have,
    \begin{align*}
    \mathbb{E}\left[R_{\cA,\bnu'}(T)\right] \geq \frac{1}{144}\mathbb{E}_{\bnu'}\left[N_1\right]  + \frac{1}{48} T^{\frac{2}{3}} - \frac{1}{96} T^{\frac{1}{3}} \s{ \mathbb{E}_{\bnu'}\left[N_1\right]} 
    \end{align*}
    If $\mathbb{E}_{\bnu'}\left[N_1\right]\geq T^{2/3}/16$, then by~\eqref{eq:lbalter}, we have,
    \begin{align*}
    \mathbb{E}\left[R_{\cA,\bnu'}(T)\right] \geq \frac{1}{144}\mathbb{E}_{\bnu'}\left[N_1\right] \geq \frac{1}{2304} T^{\frac{2}{3}} 
    \end{align*}
    Else, we have,
    \begin{align*}
    \mathbb{E}\left[R_{\cA,\bnu'}(T)\right] &\geq \frac{1}{144}\mathbb{E}_{\bnu'}\left[N_1\right]  + \frac{1}{48} T^{\frac{2}{3}} - \frac{1}{96} T^{\frac{1}{3}} \s{ \mathbb{E}_{\bnu'}\left[N_1\right]}  \\
        &\geq \frac{1}{48} T^{\frac{2}{3}} - \frac{1}{96} T^{\frac{1}{3}} \frac{1}{4} T^{\frac{1}{3}} \\
        &\geq \frac{1}{2304} T^{\frac{2}{3}} 
    \end{align*}

\end{proof}

==> appendices/app_misc.tex <==
\section{Miscellaneous}\label{app:misc}

\subsection{Explicit expression for the relative loss of a combinatorial arm}

For a given combinatorial arm $(k,l)$, we have explicitly the following 4 cases,
\begin{align*}
    \clstar{k}{l}=\begin{cases}
    \max_{i\in\{1,2\}}\lstar{i}{k} \qquad \text{if}~~\loss{1}{k}\leq \loss{1}{l}~\&~ \loss{2}{k}\leq \loss{2}{l}\,,\\
    \max_{i\in\{1,2\}}\lstar{t}{l} \qquad \text{if}~~\loss{1}{k}\geq \loss{1}{l}~\&~ \loss{2}{k}\geq \loss{2}{l}\footnotemark\,, \\
    \min_{j\in \{k,l\}}\max_{i\in\{1,2\}}\lstar{i}{j} \qquad \text{if}~~(\lstar{1}{k}-\lstar{2}{k})(\lstar{1}{l}-\lstar{2}{l}) >0\,,\\
    \dfrac{\lstar{1}{k}\lstar{2}{l}-\lstar{1}{l}\lstar{2}{k}}{\lstar{1}{k}+\lstar{2}{l}-\lstar{1}{l}-\lstar{2}{k}} \qquad \text{otherwise}\,,
    \end{cases}
\end{align*}
where the first three cases actually only depends on a single arm.\footnotetext{With two equalities not attained simultaneously.}


==> appendices/app_notations.tex <==
%!TEX root = ../main.tex
\section{Notation}\label{app:notations}

We recall and resemble the important notation in this section.

\begin{table}[h]
	\centering
	\caption{Table of notation}
	\begin{tabular}{@{}l|l@{}}
		\toprule
		\thead{Notation} & \thead{Meaning} \\ \midrule
		$K$ & number of arms \\
        $\dist{i}{k}$ & the $i$-th loss distribution for the $k$-th arm \\
        $\loss{i}{k}$ & $\mathbb{E}[\dist{i}{k}]$ \\
        $\bloss{i}$ & the vector loss of arm $i$ \\
        $\star_i$ & the set of the arms with the least $i$-th loss \\
        $\bLoss{\cA}$ & the cumulative loss of algorithm $\cA$ \\
        $\Loss{i}{\cA}$ & the cumulative $i$-th loss of algorithm $\cA$ \\
        $\bomega^\star$ & the optimal weight of arm pulls \\
        $R_\cA(T)$ & regret \\
        $\lstar{i}{k}$ & the $i$-th loss relative to $\star_i$ \\
        $\clstar{k}{l}$ & the minimum relative loss of the combinatorial arm $(k,l)$ \\
        $\hclstar{k}{l}$ & the empirical minimum relative loss of the combinatorial arm $(k,l)$ \\
        $\hwlstar{\bomega}$ & the empirical loss of weight $\bomega$ relative to $\star$ \\
        $\hhwlstar{\bomega}$ & The empirical loss of weight $\bomega$ relative to $\hat{\star}$ \\
        $\Delta = \min_{i, \loss{i}{k}-\loss{i}{l}>0} \loss{i}{k}-\loss{i}{l}$ & the minimum positive loss gap between any two arms \\
		\bottomrule
	\end{tabular}
\end{table}


==> sections/7_broader_impact.tex <==
\section*{Broader Impact}

This work could have impacts in two ways: First, specific applications could adopt more involved versions of the algorithms proposed in this work to ensure the entity fairness. Second, it could provide some intuition in understanding the regret scale if we are to compromise to ensure entity fairness.
